Cost Effective MLaaS Federation: A Combinatorial Reinforcement Learning Approach

With the advancement of deep learning techniques, major cloud providers and niche machine learning service providers start to offer their cloud-based machine learning tools, also known as machine learning as a service (MLaaS), to the public. According to our measurement, for the same task, these MLaaSes from different providers have varying performance due to the proprietary datasets, models, etc. Federating different MLaaSes together allows us to improve the analytic performance further. However, naively aggregating results from different MLaaSes not only incurs significant momentary cost but also may lead to sub-optimal performance gain due to the introduction of possible false-positive results. In this paper, we propose Armol, a framework to federate the right selection of MLaaS providers to achieve the best possible analytic performance. We first design a word grouping algorithm to unify the output labels across different providers. We then present a deep combinatorial reinforcement learning based-approach to maximize the accuracy while minimizing the cost. The predictions from the selected providers are then aggregated together using carefully chosen ensemble strategies. The real-world trace-driven evaluation further demonstrates that Armol is able to achieve the same accuracy results with $67\%$ less inference cost.

==> sections/ensemble.tex <==
% \section{Ensemble Strategy} \label{ensemble}
% The object detection cloud services output different inference results for the same image. Fig.~\ref{fig:differentproviders} illustrates the results of AWS, Azure and Google Cloud on sample images. As can be seen from Fig.~\ref{fig:differentproviders}, a single cloud service has low inference accuracy while the ensemble of multiple cloud services reaches excellent performance. Therefore, based on the measurement results in Section \ref{measurement}, we propose an ensemble strategy for inference results of object detection cloud services, which is divided into two steps: voting and fusion. The inference accuracy after ensemble is evaluated on COCO Val 2017. 

% \textbf{Voting methods.} \cite{DBLP:conf/ecai/Casado-GarciaH20} devised three voting methods to ensemble the output of object detection models, namely ``Affirmative", ``Consensus" and ``Unanimous". To conduct the voting methods, we preprocess the inference results and classify the detections. Assume we adopt object detection services from $N$ clouds, we group the detections on an image into $G = [g_1, g_2, ..., g_r]$, where $g_i, i \in \{1, 2,..., r\}$ is a list of detections and $r$ represents the total number of objects detected by $N$ cloud service providers. For detections $d_i, d_j \in g_i$, they must confirm that $IoU(b_i, b_j) > 0.5$ and $l_i = l_j$. $IoU(a, b)$ is calculated by dividing the area of intersection between box $a$ and box $b$ by the area of union between $a$ and $b$. Then we adjust the three voting methods to our work, which are described as follows.
% \begin{itemize}
%     \item Affirmative. All groups in $G$ are kept in this method. This means that whenever one of the cloud services produces a detection says that a region contains an object, the detection is considered as valid.
%     \item Consensus. In this method, only the groups with  a size greater than $N/2$ are kept. This means that the majority of the cloud must agree that a region contains an object.
%     \item Unanimous. In this method, only the groups whose size is equal to $N$ are kept. This means that all the object detection cloud services must agree to consider that a region contains an object.
% \end{itemize}

% We evaluate the above voting methods on COCO Val 2017 in Table.~\ref{mapwdvf}. The three cloud service providers are denoted as $M_1$, $M_2$ and $M_3$. We find that the predictions are complementary rather than duplicated, for the object detection cloud services. Thus,  under all cloud service combinations, the ``Affirmative" strategy shows the highest mAP among the three methods. 

% \textbf{Fusion Methods.} A group of boxes is kept in the ``Unanimous" strategy. However, boxes in a group repeatedly express an object. To reduce the useless boxes in a group, Non-Maximum Suppression(NMS) \cite{hosang2017learning}, Soft-NMS \cite{bodla2017soft}, NMW \cite{zhou2017cad}, Fusion \cite{wei2018fusion} and Weighted Boxes Fusion (WBF) \cite{solovyev2019weighted} are proposed. We calculated the mAP of COCO Val 2017 under the above methods and show our results in Table.~\ref{mapwdvf}, where Naive means no fusion methods are used. Naive, NMS, Soft-NMS and WBF have different effects under different combinations of cloud services, and it is difficult to distinguish which method is the best. 

% \begin{table*}[t]
% \caption{mAP with different combinations, voting strategies and fusion methods}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
%  \textbf{Voting Strategy} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{Naive} & \textbf{NMS} & \textbf{Soft-NMS} & \textbf{WBF}\\
% \hline
%  \multirow{4}{4em}{\textbf{Affirmative}} & 1 & 1 & 0 & 21.58 & 18.26 & 21.58 & 20.29 \\
% \cline{2-8}
%   & 1 & 0 & 1 & 20.75 & \textbf{20.14} & 20.75 & 21.15 \\
% \cline{2-8}
%   & 0 & 1 & 1 & 18.57 & 18.36 & 18.57 & 19.91 \\
% \cline{2-8}
%   & 1 & 1 & 1 & \textbf{22.11} & 19.01 & \textbf{22.11} & \textbf{22.05} \\
% \hline
% \multirow{4}{4em}{\textbf{Consensus}} & 1 & 1 & 0 & 13.33 & 11.89 & 13.34 & 13.22 \\
% \cline{2-8}
%   & 1 & 0 & 1 & 12.89 & 13.20 & 12.89 & 13.55 \\
% \cline{2-8}
%   & 0 & 1 & 1 & 11.59 & 11.16 & 11.59 & 12.46 \\
% \cline{2-8}
%   & 1 & 1 & 1 & 16.48 & 15.26 & 16.48 & 17.26 \\
% \hline
% \multirow{4}{4em}{\textbf{Unanimous}} & 1 & 1 & 0 & 13.24 & 11.81 & 13.24 & 13.14 \\
% \cline{2-8}
%   & 1 & 0 & 1 & 12.76 & 13.08 & 12.76 & 13.43 \\
% \cline{2-8}
%   & 0 & 1 & 1 & 11.48 & 11.06 & 11.48 & 12.34 \\
% \cline{2-8}
%   & 1 & 1 & 1 & 10.52 & 9.79 & 10.52 & 11.01 \\
% \hline
% \end{tabular}
% \label{mapwdvf}
% \end{center}
% \end{table*}

% This section is described on the right half of Fig.~\ref{frameworkoverview}, where we use the ``Affirmative" strategy in the voting step, and compare the above four bounding boxes fusion approaches by mAP.
